Bridging the Gap between Stochastic Gradient MCMC and Stochastic Optimization

Stochastic gradient Markov chain Monte Carlo (SG-MCMC) methods are Bayesian analogs to popular stochastic optimization methods; however, this connection is not well studied. We explore this relationship by applying simulated annealing to an SGMCMC algorithm. Furthermore, we extend recent SG-MCMC methods with two key components: i) adaptive preconditioners (as in ADAgrad or RMSprop), and ii) adaptive element-wise momentum weights. The zero-temperature limit gives a novel stochastic optimization method with adaptive element-wise momentum weights, while conventional optimization methods only have a shared, static momentum weight. Under certain assumptions, our theoretical analysis suggests the proposed simulated annealing approach converges close to the global optima. Experiments on several deep neural network models show state-of-the-art results compared to related stochastic optimization algorithms.

==> Definitions.tex <==
\newcommand{\eat}[1]{}

\newcommand{\Cy}{\Ccal_y}
\renewcommand{\l}{\boldsymbol{\ell}}
\renewcommand{\S}
{\!\!\,\includegraphics[height=1em]{figs/arcsinh}\!\!}
\def\Gt{\widetilde{G}}
\def\ah{\widehat{a}}
\def\ahb{\mathbf{\ah}}
\def\at{\widetilde{a}}
\def\atb{\mathbf{\at}}
\def\yh{\widehat{y}}
\def\yt{\widetilde{y}}
\def\ytb{\mathbf{\yt}}
\def\yhb{\mathbf{\yh}}
\def\zh{\widehat{z}}
\def\zt{\widetilde{z}}
\def\ztb{\mathbf{\zt}}
\def\zhb{\mathbf{\zh}}
\def\g{\mathbf{g}}
\def\bah{\mathbf{\widehat{a}}}
\RequirePackage{latexsym}
\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

\definecolor{magenta}{cmyk}{0,1,0,0}
\definecolor{mygreen}{rgb}{.1,1,.1}
\newcommand{\Magenta}[1]{\color{magenta}{#1}\color{black}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
%\newcommand{\Green}[1]{\color{OliveGreen}{#1}}
\newcommand{\Green}[1]{\textcolor{mygreen}{#1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\Orange}[1]{\textcolor{orange}{#1}}
\newcommand{\Brown}[1]{\textcolor{brown}{#1}}
\newcommand{\Ref}[1]{\hfill\Green{[#1]}}
\DeclareMathOperator{\arginf}{arg\,inf}
%\newcommand{\alert}[1]{\Red{\bf {#1}}}

\newcommand{\rmd}{\mathrm{d}} % use italics only for variable

\newcommand{\Tr}{^\mathsf{T}} % sf looks nicer than rm


%%% MW %%%%

\newcommand{\mnote}[1]{{\bf\large *}\marginpar{\Magenta{#1}}}
\newcommand{\dnote}[1]{{\bf\large +}\marginpar{\tiny#1}}
\ifx\note\undefined
\newcommand{\note}[1]{{\bf \Magenta{#1}}}
\else
\renewcommand{\note}[1]{{\bf \Magenta{#1}}}
\fi

\def\x{\mathbf{x}}
\def\a{\mathbf{a}}
\def\y{\mathbf{y}}
\def\z{\mathbf{z}}
\def\w{\mathbf{w}}
\def\t{\boldsymbol{\theta}}
\def\R{\mathbb{R}}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\ab}{\mathbf{a}}
\DeclareMathOperator{\bb}{\mathbf{b}}
\DeclareMathOperator{\cbb}{\mathbf{c}}
\DeclareMathOperator{\db}{\mathbf{d}}
\DeclareMathOperator{\eb}{\mathbf{e}}
\DeclareMathOperator{\fb}{\mathbf{f}}
\DeclareMathOperator{\gb}{\mathbf{g}}
\DeclareMathOperator{\hb}{\mathbf{h}}
\DeclareMathOperator{\ib}{\mathbf{i}}
\DeclareMathOperator{\jb}{\mathbf{j}}
\DeclareMathOperator{\kb}{\mathbf{k}}
\DeclareMathOperator{\lb}{\mathbf{l}}
\DeclareMathOperator{\mb}{\mathbf{m}}
\DeclareMathOperator{\nbb}{\mathbf{n}}
\DeclareMathOperator{\ob}{\mathbf{o}}
\DeclareMathOperator{\pb}{\mathbf{p}}
\DeclareMathOperator{\qb}{\mathbf{q}}
\DeclareMathOperator{\rb}{\mathbf{r}}
\DeclareMathOperator{\sbb}{\mathbf{s}}
\DeclareMathOperator{\tb}{\mathbf{t}}
\DeclareMathOperator{\ub}{\mathbf{u}}
\DeclareMathOperator{\vb}{\mathbf{v}}
\DeclareMathOperator{\wb}{\mathbf{w}}
\DeclareMathOperator{\xb}{\mathbf{x}}
 \DeclareMathOperator{\yb}{\mathbf{y}}
\DeclareMathOperator{\zb}{\mathbf{z}}



\DeclareMathOperator{\atilde}{\tilde{\ab}}
\DeclareMathOperator{\btilde}{\tilde{\bb}}
\DeclareMathOperator{\ctilde}{\tilde{\cb}}
\DeclareMathOperator{\dtilde}{\tilde{\db}}
\DeclareMathOperator{\etilde}{\tilde{\eb}}
\DeclareMathOperator{\ftilde}{\tilde{\fb}}
\DeclareMathOperator{\gtilde}{\tilde{\gb}}
\DeclareMathOperator{\htilde}{\tilde{\hb}}
\DeclareMathOperator{\itilde}{\tilde{\ib}}
\DeclareMathOperator{\jtilde}{\tilde{\jb}}
\DeclareMathOperator{\ktilde}{\tilde{\kb}}
\DeclareMathOperator{\ltilde}{\tilde{\lb}}
\DeclareMathOperator{\mtilde}{\tilde{\mb}}
\DeclareMathOperator{\ntilde}{\tilde{\nbb}}
\DeclareMathOperator{\otilde}{\tilde{\ob}}
%
\DeclareMathOperator{\qtilde}{\tilde{\qb}}
\DeclareMathOperator{\rtilde}{\tilde{\rb}}
\DeclareMathOperator{\stilde}{\tilde{\sbb}}
\DeclareMathOperator{\ttilde}{\tilde{\tb}}
\DeclareMathOperator{\utilde}{\tilde{\ub}}
\DeclareMathOperator{\vtilde}{\tilde{\vb}}
\DeclareMathOperator{\wtilde}{\tilde{\wb}}
\DeclareMathOperator{\xtilde}{\tilde{\xb}}
\DeclareMathOperator{\ytilde}{\tilde{\yb}}
\DeclareMathOperator{\ztilde}{\tilde{\zb}}

\DeclareMathOperator{\abar}{\bar{\ab}}
\DeclareMathOperator{\bbar}{\bar{\bb}}
\DeclareMathOperator{\cbar}{\bar{\cb}}
\DeclareMathOperator{\dbar}{\bar{\db}}
\DeclareMathOperator{\ebar}{\bar{\eb}}
\DeclareMathOperator{\fbar}{\bar{\fb}}
\DeclareMathOperator{\gbar}{\bar{\gb}}
\DeclareMathOperator{\hbbar}{\bar{\hb}}
\DeclareMathOperator{\ibar}{\bar{\ib}}
\DeclareMathOperator{\jbar}{\bar{\jb}}
\DeclareMathOperator{\kbar}{\bar{\kb}}
\DeclareMathOperator{\lbar}{\bar{\lb}}
\DeclareMathOperator{\mbar}{\bar{\mb}}
\DeclareMathOperator{\nbar}{\bar{\nbb}}
\DeclareMathOperator{\obar}{\bar{\ob}}
\DeclareMathOperator{\pbar}{\bar{\pb}}
\DeclareMathOperator{\qbar}{\bar{\qb}}
\DeclareMathOperator{\rbar}{\bar{\rb}}
\DeclareMathOperator{\sbar}{\bar{\sbb}}
\DeclareMathOperator{\tbar}{\bar{\tb}}
\DeclareMathOperator{\ubar}{\bar{\ub}}
\DeclareMathOperator{\vbar}{\bar{\vb}}
\DeclareMathOperator{\wbar}{\bar{\wb}}
\DeclareMathOperator{\xbar}{\bar{\xb}}
\DeclareMathOperator{\ybar}{\bar{\yb}}
\DeclareMathOperator{\zbar}{\bar{\zb}}

\DeclareMathOperator{\Ab}{\mathbf{A}}
\DeclareMathOperator{\Bb}{\mathbf{B}}
\DeclareMathOperator{\Cb}{\mathbf{C}}
\DeclareMathOperator{\Db}{\mathbf{D}}
\DeclareMathOperator{\Eb}{\mathbf{E}}
\DeclareMathOperator{\Fb}{\mathbf{F}}
\DeclareMathOperator{\Gb}{\mathbf{G}}
\DeclareMathOperator{\Hb}{\mathbf{H}}
\DeclareMathOperator{\Ib}{\mathbf{I}}
\DeclareMathOperator{\Jb}{\mathbf{J}}
\DeclareMathOperator{\Kb}{\mathbf{K}}
\DeclareMathOperator{\Lb}{\mathbf{L}}
\DeclareMathOperator{\Mb}{\mathbf{M}}
\DeclareMathOperator{\Nb}{\mathbf{N}}
\DeclareMathOperator{\Ob}{\mathbf{O}}
\DeclareMathOperator{\Pb}{\mathbf{P}}
\DeclareMathOperator{\Qb}{\mathbf{Q}}
\DeclareMathOperator{\Rb}{\mathbf{R}}
\DeclareMathOperator{\Sbb}{\mathbf{S}}
\DeclareMathOperator{\Tb}{\mathbf{T}}
\DeclareMathOperator{\Ub}{\mathbf{U}}
\DeclareMathOperator{\Vb}{\mathbf{V}}
\DeclareMathOperator{\Wb}{\mathbf{W}}
\DeclareMathOperator{\Xb}{\mathbf{X}}
\DeclareMathOperator{\Yb}{\mathbf{Y}}
\DeclareMathOperator{\Zb}{\mathbf{Z}}

\DeclareMathOperator{\Abar}{\bar{A}}
\DeclareMathOperator{\Bbar}{\bar{B}}
\DeclareMathOperator{\Cbar}{\bar{C}}
\DeclareMathOperator{\Dbar}{\bar{D}}
\DeclareMathOperator{\Ebar}{\bar{E}}
\DeclareMathOperator{\Fbar}{\bar{F}}
\DeclareMathOperator{\Gbar}{\bar{G}}
\DeclareMathOperator{\Hbar}{\bar{H}}
\DeclareMathOperator{\Ibar}{\bar{I}}
\DeclareMathOperator{\Jbar}{\bar{J}}
\DeclareMathOperator{\Kbar}{\bar{K}}
\DeclareMathOperator{\Lbar}{\bar{L}}
\DeclareMathOperator{\Mbar}{\bar{M}}
\DeclareMathOperator{\Nbar}{\bar{N}}
\DeclareMathOperator{\Obar}{\bar{O}}
\DeclareMathOperator{\Pbar}{\bar{P}}
\DeclareMathOperator{\Qbar}{\bar{Q}}
\DeclareMathOperator{\Rbar}{\bar{R}}
\DeclareMathOperator{\Sbar}{\bar{S}}
\DeclareMathOperator{\Tbar}{\bar{T}}
\DeclareMathOperator{\Ubar}{\bar{U}}
\DeclareMathOperator{\Vbar}{\bar{V}}
\DeclareMathOperator{\Wbar}{\bar{W}}
\DeclareMathOperator{\Xbar}{\bar{X}}
\DeclareMathOperator{\Ybar}{\bar{Y}}
\DeclareMathOperator{\Zbar}{\bar{Z}}

\DeclareMathOperator{\Abbar}{\bar{\Ab}}
\DeclareMathOperator{\Bbbar}{\bar{\Bb}}
\DeclareMathOperator{\Cbbar}{\bar{\Cb}}
\DeclareMathOperator{\Dbbar}{\bar{\Db}}
\DeclareMathOperator{\Ebbar}{\bar{\Eb}}
\DeclareMathOperator{\Fbbar}{\bar{\Fb}}
\DeclareMathOperator{\Gbbar}{\bar{\Gb}}
\DeclareMathOperator{\Hbbar}{\bar{\Hb}}
\DeclareMathOperator{\Ibbar}{\bar{\Ib}}
\DeclareMathOperator{\Jbbar}{\bar{\Jb}}
\DeclareMathOperator{\Kbbar}{\bar{\Kb}}
\DeclareMathOperator{\Lbbar}{\bar{\Lb}}
\DeclareMathOperator{\Mbbar}{\bar{\Mb}}
\DeclareMathOperator{\Nbbar}{\bar{\Nb}}
\DeclareMathOperator{\Obbar}{\bar{\Ob}}
\DeclareMathOperator{\Pbbar}{\bar{\Pb}}
\DeclareMathOperator{\Qbbar}{\bar{\Qb}}
\DeclareMathOperator{\Rbbar}{\bar{\Rb}}
\DeclareMathOperator{\Sbbar}{\bar{\Sb}}
\DeclareMathOperator{\Tbbar}{\bar{\Tb}}
\DeclareMathOperator{\Ubbar}{\bar{\Ub}}
\DeclareMathOperator{\Vbbar}{\bar{\Vb}}
\DeclareMathOperator{\Wbbar}{\bar{\Wb}}
\DeclareMathOperator{\Xbbar}{\bar{\Xb}}
\DeclareMathOperator{\Ybbar}{\bar{\Yb}}
\DeclareMathOperator{\Zbbar}{\bar{\Zb}}

\DeclareMathOperator{\Ahat}{\widehat{A}}
\DeclareMathOperator{\Bhat}{\widehat{B}}
\DeclareMathOperator{\Chat}{\widehat{C}}
\DeclareMathOperator{\Dhat}{\widehat{D}}
\DeclareMathOperator{\Ehat}{\widehat{E}}
\DeclareMathOperator{\Fhat}{\widehat{F}}
\DeclareMathOperator{\Ghat}{\widehat{G}}
\DeclareMathOperator{\Hhat}{\widehat{H}}
\DeclareMathOperator{\Ihat}{\widehat{I}}
\DeclareMathOperator{\Jhat}{\widehat{J}}
\DeclareMathOperator{\Khat}{\widehat{K}}
\DeclareMathOperator{\Lhat}{\widehat{L}}
\DeclareMathOperator{\Mhat}{\widehat{M}}
\DeclareMathOperator{\Nhat}{\widehat{N}}
\DeclareMathOperator{\Ohat}{\widehat{O}}
\DeclareMathOperator{\Phat}{\widehat{P}}
\DeclareMathOperator{\Qhat}{\widehat{Q}}
\DeclareMathOperator{\Rhat}{\widehat{R}}
\DeclareMathOperator{\Shat}{\widehat{S}}
\DeclareMathOperator{\That}{\widehat{T}}
\DeclareMathOperator{\Uhat}{\widehat{U}}
\DeclareMathOperator{\Vhat}{\widehat{V}}
\DeclareMathOperator{\What}{\widehat{W}}
\DeclareMathOperator{\Xhat}{\widehat{X}}
\DeclareMathOperator{\Yhat}{\widehat{Y}}
\DeclareMathOperator{\Zhat}{\widehat{Z}}

\DeclareMathOperator{\Abhat}{\widehat{\Ab}}
\DeclareMathOperator{\Bbhat}{\widehat{\Bb}}
\DeclareMathOperator{\Cbhat}{\widehat{\Cb}}
\DeclareMathOperator{\Dbhat}{\widehat{\Db}}
\DeclareMathOperator{\Ebhat}{\widehat{\Eb}}
\DeclareMathOperator{\Fbhat}{\widehat{\Fb}}
\DeclareMathOperator{\Gbhat}{\widehat{\Gb}}
\DeclareMathOperator{\Hbhat}{\widehat{\Hb}}
\DeclareMathOperator{\Ibhat}{\widehat{\Ib}}
\DeclareMathOperator{\Jbhat}{\widehat{\Jb}}
\DeclareMathOperator{\Kbhat}{\widehat{\Kb}}
\DeclareMathOperator{\Lbhat}{\widehat{\Lb}}
\DeclareMathOperator{\Mbhat}{\widehat{\Mb}}
\DeclareMathOperator{\Nbhat}{\widehat{\Nb}}
\DeclareMathOperator{\Obhat}{\widehat{\Ob}}
\DeclareMathOperator{\Pbhat}{\widehat{\Pb}}
\DeclareMathOperator{\Qbhat}{\widehat{\Qb}}
\DeclareMathOperator{\Rbhat}{\widehat{\Rb}}
\DeclareMathOperator{\Sbhat}{\widehat{\Sb}}
\DeclareMathOperator{\Tbhat}{\widehat{\Tb}}
\DeclareMathOperator{\Ubhat}{\widehat{\Ub}}
\DeclareMathOperator{\Vbhat}{\widehat{\Vb}}
\DeclareMathOperator{\Wbhat}{\widehat{\Wb}}
\DeclareMathOperator{\Xbhat}{\widehat{\Xb}}
\DeclareMathOperator{\Ybhat}{\widehat{\Yb}}
\DeclareMathOperator{\Zbhat}{\widehat{\Zb}}

\DeclareMathOperator{\Acal}{\mathcal{A}}
\DeclareMathOperator{\Bcal}{\mathcal{B}}
\DeclareMathOperator{\Ccal}{\mathcal{C}}
\DeclareMathOperator{\Dcal}{\mathcal{D}}
\DeclareMathOperator{\Ecal}{\mathcal{E}}
\DeclareMathOperator{\Fcal}{\mathcal{F}}
\DeclareMathOperator{\Gcal}{\mathcal{G}}
\DeclareMathOperator{\Hcal}{\mathcal{H}}
\DeclareMathOperator{\Ical}{\mathcal{I}}
\DeclareMathOperator{\Jcal}{\mathcal{J}}
\DeclareMathOperator{\Kcal}{\mathcal{K}}
\DeclareMathOperator{\Lcal}{\mathcal{L}}
\DeclareMathOperator{\Mcal}{\mathcal{M}}
\DeclareMathOperator{\Ncal}{\mathcal{N}}
\DeclareMathOperator{\Ocal}{\mathcal{O}}
\DeclareMathOperator{\Pcal}{\mathcal{P}}
\DeclareMathOperator{\Qcal}{\mathcal{Q}}
\DeclareMathOperator{\Rcal}{\mathcal{R}}
\DeclareMathOperator{\Scal}{\mathcal{S}}
\DeclareMathOperator{\Tcal}{\mathcal{T}}
\DeclareMathOperator{\Ucal}{\mathcal{U}}
\DeclareMathOperator{\Vcal}{\mathcal{V}}
\DeclareMathOperator{\Wcal}{\mathcal{W}}
\DeclareMathOperator{\Xcal}{\mathcal{X}}
\DeclareMathOperator{\Ycal}{\mathcal{Y}}
\DeclareMathOperator{\Zcal}{\mathcal{Z}}

\DeclareMathOperator{\Atilde}{\widetilde{A}}
\DeclareMathOperator{\Btilde}{\widetilde{B}}
\DeclareMathOperator{\Ctilde}{\widetilde{C}}
\DeclareMathOperator{\Dtilde}{\widetilde{D}}
\DeclareMathOperator{\Etilde}{\widetilde{E}}
\DeclareMathOperator{\Ftilde}{\widetilde{F}}
\DeclareMathOperator{\Gtilde}{\widetilde{G}}
\DeclareMathOperator{\Htilde}{\widetilde{H}}
\DeclareMathOperator{\Itilde}{\widetilde{I}}
\DeclareMathOperator{\Jtilde}{\widetilde{J}}
\DeclareMathOperator{\Ktilde}{\widetilde{K}}
\DeclareMathOperator{\Ltilde}{\widetilde{L}}
\DeclareMathOperator{\Mtilde}{\widetilde{M}}
\DeclareMathOperator{\Ntilde}{\widetilde{N}}
\DeclareMathOperator{\Otilde}{\widetilde{O}}
\DeclareMathOperator{\Ptilde}{\widetilde{P}}
\DeclareMathOperator{\Qtilde}{\widetilde{Q}}
\DeclareMathOperator{\Rtilde}{\widetilde{R}}
\DeclareMathOperator{\Stilde}{\widetilde{S}}
\DeclareMathOperator{\Ttilde}{\widetilde{T}}
\DeclareMathOperator{\Utilde}{\widetilde{U}}
\DeclareMathOperator{\Vtilde}{\widetilde{V}}
\DeclareMathOperator{\Wtilde}{\widetilde{W}}
\DeclareMathOperator{\Xtilde}{\widetilde{X}}
\DeclareMathOperator{\Ytilde}{\widetilde{Y}}
\DeclareMathOperator{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers

\DeclareMathOperator{\one}{\mathbf{1}}  % Identity
\DeclareMathOperator{\zero}{\mathbf{0}} % Zero

\DeclareMathOperator*{\mini}{\mathop{\mathrm{minimize}}}
\DeclareMathOperator*{\maxi}{\mathop{\mathrm{maximize}}}
\DeclareMathOperator*{\argmin}{\mathop{\mathrm{argmin}}}
\DeclareMathOperator*{\argsup}{\mathop{\mathrm{argsup}}}
\DeclareMathOperator*{\arcsinh}{\mathop{\mathrm{arcsinh}}}
\DeclareMathOperator*{\limit}{\mathop{\mathrm{limit}}}
\DeclareMathOperator*{\argmax}{\mathop{\mathrm{argmax}}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}
\DeclareMathOperator{\diag}{diag}

%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{{\bm{\Theta}}}
\newcommand{\thetab}{{\bm{\theta}}}
\newcommand{\xib}{{\bm{\xi}}}
\newcommand{\Xib}{{\bm{\Xi}}}
\newcommand{\zetab}{{\bm{\zeta}}}
\newcommand{\alphab}{{\bm{\alpha}}}
\newcommand{\taub}{{\bm{\tau}}}
\newcommand{\etab}{{\bm{\eta}}}


\DeclareMathOperator{\alphahat}{\widehat{\alpha}}
%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi
\ifx\example\undefined
\newtheorem{example}{Example}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}[theorem]{Definition}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\factoid\undefined
\newtheorem{factoid}[theorem]{Fact}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

\newcommand{\ea}{\emph{et al. }}
\newcommand{\eg}{\emph{e.g. }}
\newcommand{\ie}{\emph{i.e., }}

\newcommand{\vishy}[1]{{\bf[#1--VISHY]}}
\newcommand{\tim}[1]{{\bf[#1 --TIM]}}

%Logic
%\newcommand{\implies}{\Rightarrow}
%\newcommand{\iff}{\Leftrightarrow}
\newcommand{\goesto}{\rightarrow}
\newcommand{\suchthat}{\ensuremathmode{\text{ such that }}}
\newcommand{\st}{\suchthat}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

% upright names for matrices --don't use for single-letter function names!
\newcommand{\A}{\mathbf{A}}
\newcommand{\As}{\mathbf{A}^{\!\!*}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Bs}{\mathbf{B}^{*}}

% p and variants
\newcommand{\p}{\mathbf{p}}
\newcommand{\pp}{\p^{\prime}}
\newcommand{\ps}{\p^*}
\newcommand{\po}{\p_0}
\newcommand{\pos}{\p_{0}^{*}}
\newcommand{\poi}{[\p_{0}]_i}
\newcommand{\pii}{\p_{i}}
\newcommand{\pip}{\p_{i}^{\prime}}
\newcommand{\pis}{\p_{i}^{*}}
\newcommand{\pBar}{\bar{\p}}
\newcommand{\pohat}{\widehat{\p}_0}
\newcommand{\phat}{\widehat{\p}}
\newcommand{\psBar}{\bar{\p}^{*}}
\newcommand{\pbb}{\p_{\bb}}

% mu and variants
\newcommand{\mub}{{\bm{\mu}}}
\newcommand{\ms}{\m^{*}}
\newcommand{\mo}{\m_0}
\newcommand{\mh}{\widehat{\m}}
\newcommand{\mBar}{\bar{\m}}
\newcommand{\msBar}{\bar{\m}^{*}}

% Bold mu_B
\newcommand{\mB}{\m_{\B}}
\newcommand{\mBBar}{\bar{\m}_{\B}}
% mu_1
\newcommand{\mone}{\mu_{\mathbf{1}}}
\newcommand{\mones}{\mu_{\mathbf{1}}^{*}}
\newcommand{\monesBar}{\bar{\mu}^{*}_\mathbf{1}}

% q and variants
\newcommand{\q}{\mathbf{q}}
\newcommand{\qs}{\q^{*}}
\newcommand{\qii}{\q_{i}}

% b and variants
\newcommand{\bone}{\mathbf{b_1}}
%\newcommand{\bone}{\ones}

% c and variants
\newcommand{\cs}{\cbb^{*}}

% Functions
\newcommand{\Fs}{F^{*}}
\newcommand{\Gs}{G^{*}}
\newcommand{\Hs}{H^{*}}
\newcommand{\fsi}{f_{i}^{*}}

% Dual Spaces
\DeclareMathOperator{\Xcals}{\Xcal^{*}}
\DeclareMathOperator{\Mcals}{\Mcal^{*}}

% set and domain concepts
\DeclareMathOperator{\ri}{\mathrm{ri}}      % Relative interior
\DeclareMathOperator{\intr}{\mathrm{int}}   % Interior
\DeclareMathOperator{\bd}{\mathrm{bdry}}      % Boundary (see RocWet98)
\DeclareMathOperator{\dom}{\mathrm{dom}}    % Effective Domain
\DeclareMathOperator{\epi}{\mathrm{epi}}    % Epigraph
\DeclareMathOperator{\ran}{\mathrm{range}}  % Range of an operator

\newcommand{\by}{\times}

% gradient: \grad{F}{\m}
\newcommand{\grad}[2]{\nabla #1 \left( #2 \right) }
\newcommand{\hess}[2]{\nabla^2 #1 \left( #2 \right) }
\newcommand{\grd}{\nabla} % simpler version!
\newcommand{\breg}[1]{\Delta #1} % Bregman divergence

% subgradient: \subgrad{F}{\m}
\newcommand{\subgrad}[2]{\partial #1 \left( #2 \right) }
% subdiferential
\newcommand{\subdiff}{\partial}

% Vector of all ones
\newcommand{\ones}{\eb}

% Sum from i equal 1 to n
\newcommand{\sumin}{\sum_{i=1}^{n}}

% Deformed logarithm wrt \phi
\newcommand{\lphi}{\log_{\phi}}

% function k_{\phi}
\newcommand{\kphi}{k_{\phi}}

% reparam for dual log
\newcommand{\phib}{\phi^{\bullet}}
\newcommand{\psib}{\psi^{\bullet}}

% Deformed exponential wrt \phi
\newcommand{\ephi}{\exp_{\phi}}

% One over deformed exponential wrt \phi
\newcommand{\ephib}{\exp^{\bullet}_{\phi}}

% Gradient of deformed exponential wrt \phi
\newcommand{\ephip}{\nabla_{x} \exp_{\phi}}

% Gradient of t-exponential wrt \phi
\newcommand{\ephit}{\nabla_{x} \exp_{t}}

% Deformed logarithm wrt \psi
\newcommand{\lpsi}{\log_{\psi}}

% One over deformed logarithm wrt \psi
\newcommand{\lpsib}{\log^{\bullet}_{\psi}}
\newcommand{\lphib}{\log^{\bullet}_{\phi}}

%composition needed for conjugate--formerly combo
\newcommand{\lcirce}{\lpsi \circ \ephib}

% S and related
\newcommand{\Sp}{S_{\phi}}
\newcommand{\Sps}{S^{*}_{\phi}}
\newcommand{\smp}{s_{\phi}}
\newcommand{\smpp}{s^{\prime}_{\phi}}
\newcommand{\smps}{s^{*}_{\phi}}

% T
\newcommand{\T}{T^{*}}
\DeclareMathOperator{\tp}{\tilde{p}}
\DeclareMathOperator{\tq}{\tilde{q}}
\DeclareMathOperator{\tg}{\tilde{g}}
\DeclareMathOperator{\tmu}{\tilde{\mu}}
\DeclareMathOperator{\tthe}{\tilde{\theta}}
\DeclareMathOperator{\ttheb}{{\bf \tilde{\theta}}}
\DeclareMathOperator{\tmc}{\widehat{\Mcal}}
\DeclareMathOperator{\tv}{\tilde{v}}


\DeclareMathOperator{\Remp}{R_{\text{emp}}}

\DeclareMathOperator{\tsallis}{\text{tsallis}}

%\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
%\newcommand{\rbr}[1]{\left(#1\right)}
%\newcommand{\cbr}[1]{\left\{#1\right\}}
%\newcommand{\nbr}[1]{\left\|#1\right\|}
%\newcommand{\abr}[1]{\left|#1\right|}
\def\ah{\widehat{a}}
\def\ahb{\mathbf{\ah}}
%\newcommand{\sbr}[1]{\left[#1\right]}
%\DeclareMathOperator*{\arginf}{\mathop{\mathrm{arginf}}}
\DeclareMathOperator*{\lnm}{\mathop{\mathbf{ln}}}
\mathchardef\Theta="7102 \mathchardef\theta="7112
\newcommand{\I}{{\mathcal{I}}}
\newcommand{\tops}{{\!\top\!}}
%\newcommand{\R}{\hbox{\bf R}}
%\newcommand{\z}{{\mathbf{z}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\m}{{\mathbf{m}}}
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\renewcommand{\k}{k}
\ifx\br\undefined
\newcommand{\br}{\color{red}}
\else
\renewcommand{\br}{\color{red}}
\fi
%\newcommand{\bb}{\color{blue}}
\newcommand{\brh}{\color{red}}
\newcommand{\bbh}{\color{blue}}
\newcommand{\N}{\hbox{\bf N}}
\newcommand{\Nl}{N}
\newcommand{\Proj}{P} 
\newcommand{\Hc}{{H}}             % base hypothesis class
\def\x{{\mathbf{x}}} 
\def\X{{\mathbf{X}}} 
\def\Xr{{\rm\sf X}} 
\newcommand{\eps}{\epsilon}
\def\y{{\mathbf{y}}} 
\def\w{{\mathbf{w}}} 
\def\W{{\mathbf{W}}} 
\def\RR{{\mathbf{R}}} 
\def\NN{{\mathbf{N}}} 
\newcommand{\M}{{\boldsymbol{\mu}}}
\newcommand{\ev}{\hbox{\bf v}}
\newcommand{\EV}{\hbox{\bf V}}
\def\H{{\cal{H}}}
\def\F{{\cal{F}}}
\def\Fc{{S}}
\def\Sample{{\Z}}
\def\vc{{d}}
\def\D{{\cal{D}}} 
\def\hatD{\hat{D}} 
\def\A{\hat{A}} 
\def\B{\hat{B}} 
\def\T{\hat{T}} 
\def\G{\mathcal{G}} 
\def\P{\hat{P}} 
\newcommand{\al}{\alpha}
%\newcommand{\Fs}{{\mathcal{F}}}   % feature space
\newcommand{\AL}{{\boldsymbol \alpha}}
\newcommand{\BE}{{\boldsymbol \beta}}
\newcommand{\XI}{{\boldsymbol \xi}}
%\newcommand{\sgn}{\mbox{sgn}}
\def\one{{\mathbf{1}}}
\def\hatf{\hat{f}}
\definecolor{lila}{rgb}{0.2,0,0.5}
\definecolor{rot}{rgb}{0.8,0,0}
\definecolor{blau}{rgb}{0,0,0.5}
\definecolor{gruen}{rgb}{0,0.5,0}
\definecolor{grau}{rgb}{0.85,0.8,0.85}
\definecolor{mygreen}{rgb}{.1,1,.1}

%\definecolor{Red}{rgb}{0.75,0,0}
%\definecolor{Blue}{rgb}{0,0,0.75}
%\definecolor{Green}{rgb}{0,0.75,0}
%\definecolor{Black}{rgb}{0,0,0}
%\definecolor{Orange}{rgb}{0.9,0.5,0}

%\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
%\newcommand{\Green}[1]{\color{OliveGreen}{#1}}
%\newcommand{\Green}[1]{\textcolor{mygreen}{#1}}
%\newcommand{\Red}[1]{\textcolor{red}{#1}}
%\newcommand{\Orange}[1]{\textcolor{orange}{#1}}

\newcommand{\sign}{\mathop{\rm sign}}
%\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\tr}{\mathop{\rm tr}}
%\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\Ind}{\mathop{\rm I}}
\renewcommand{\d}{{\bf d}}
\renewcommand{\l}{\Nl}
%\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Z}{\bf Z}

\newcommand{\mg}{{\rho}}
\newcommand{\MG}{{\varrho}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\ct}{{\tilde{c}}}

%\newtheorem{example}{Example} 
%\newtheorem{remark}[example]{Remark}
%\newtheorem{theorem}[example]{Theorem} 
%\newtheorem{lemma}[example]{Lemma} 
%\newtheorem{proposition}[example]{Proposition} 
%\newtheorem{corollary}[example]{Corollary}
%\newtheorem{definition}[example]{Definition}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tit"
%%% End: 

\newcommand{\bigdot}[1]{\stackrel{\bullet}{#1}} 
\newcommand{\textc}{\color{hblue}}
\newcommand{\fgc}{\color{red}}
\newcommand{\othc}{\color{green}}
\newcommand{\bgc}{\color{black}}
\newcommand{\titc}{\bf\fgc}

%\renewcommand{{\tem}}{{\item[{\fgc $\bullet$}]}}
%\newcommand{\Ref}[1]{{\hfill\othc [#1]}}

\newcommand{\s}{\vspace*{2cm}}
\newcommand{\hs}{\vspace*{1cm}}
\ifx\bl\undefined
\newcommand{\bl}{\hspace*{0.8cm}}
\else
\renewcommand{\bl}{\hspace*{0.8cm}}
\fi
\renewcommand{\ss}{\vspace*{4cm}}
\newcommand{\fhs}{\\[2mm]}
\newcommand{\fs}{\\[4mm]}
\newcommand{\fss}{\\[8mm]}
\newcommand{\bra}[1]
       {\left. \begin{array}{c} \\[#1] \end{array} \right\} }

%\newcommand{\Lbf}{\LARGE\bf}
\newcommand{\lbf}{\large\bf}


%\newcommand{\grad}{\nabla}
\newcommand{\diff}{d\;}
%\newcommand{\qed}{$\;\;\;\Box$}
\newcommand{\equref}[1]{(\ref{#1})}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
%\newcommand{\half}{\sfrac{1}{2}}
%\newcommand{\R}{{\bf R}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
%\newcommand{\argmin}{\mbox{argmin}}
%\renewcommand{\min}{\mbox{min}}
%\renewcommand{\max}{\mbox{max}}


\newcommand{\Wc}{{\mathcal{W}}}


%\newcommand{\vect}[1]{{\bf #1}}
\newcommand{\vect}[1]{{\mbox{\boldmath $#1$}}}
\newcommand{\squiggle}[1]{{\widetilde{#1}}}
%\newcommand{\bm}[1]{{\mbox{$\boldmath#1 $}}}

\newcommand{\dat}{{\cal{X}}}
\renewcommand{\d}{\Delta}

%\newcommand{\vb}{V_B}
\newcommand{\uo}{U_1}
\newcommand{\utp}{U_{t+1}}

%\newcommand{\zero}{\vect{0}}
%\renewcommand{\one}{\vect{1}}


\newcommand{\f}{\vect{f}}
\renewcommand{\x}{\vect{x}}
\renewcommand{\u}{\vect{u}}
%\newcommand{\bb}{\vect{b}}
\renewcommand{\y}{\vect{y}}
\newcommand{\xs}{\tilde{\x}}
\newcommand{\xo}{\x_1}
\newcommand{\xt}{\x_t}
\newcommand{\xq}{\x_q}
\newcommand{\xtp}{\x_{t+1}}
\newcommand{\xtm}{\x_{t-1}}

%\newcommand{\yt}{y_t}
\newcommand{\yq}{y_q}
%\newcommand{\yh}{\hat{y}}
\newcommand{\yht}{\yh_t}

\newcommand{\mus}{\squiggle{\mu}}
\renewcommand{\m}{\vect{\mu}}
%\newcommand{\mb}{\vect{\mu}_B}
\newcommand{\mt}{\m_t}
%\newcommand{\mr}{\m^*}
%\newcommand{\mo}{\m_1}
\newcommand{\mtp}{\m_{t+1}}
\newcommand{\mtm}{\m_{t-1}}
\newcommand{\mTp}{\m_{T+1}}
%\newcommand{\ms}{\squiggle{\m}}

%\renewcommand{\o}{{\omega}}
%\newcommand{\ot}{\o_t}
%\newcommand{\otp}{\o_{t+1}}
%\newcommand{\os}{\squiggle{\o}}
%\renewcommand{\O}{\bf{\Omega}}
%\renewcommand{\O}{\bf{g(\TH)}}
%\newcommand{\M}{\bf{M}}


\renewcommand{\th}{\vect{\theta}}
\newcommand{\tht}{\th_t}
\newcommand{\tho}{\th_1}
\newcommand{\thb}{\th_B}
\newcommand{\thtp}{\th_{t+1}}
\newcommand{\thTp}{\th_{T+1}}
\newcommand{\ths}{\squiggle{\th}}
\newcommand{\thetas}{\squiggle{\theta}}
\newcommand{\thr}{\th^*}

\newcommand{\ta}{\vect{\tau}}
\renewcommand{\w}{\vect{w}}
\newcommand{\uu}{\vect{u}}
\newcommand{\dv}{\vect{d}}
\newcommand{\vv}{\vect{v}}
\newcommand{\ws}{\squiggle{\w}}
\newcommand{\Ws}{\widetilde{\W}}
\newcommand{\wo}{\w_1}
\newcommand{\wt}{\w_t}
%\newcommand{\wb}{\w_B}
\newcommand{\vt}{\vv_t}
\newcommand{\wtp}{\w_{t+1}}
\newcommand{\vtp}{\vv_{t+1}}
\newcommand{\ttheta}{\mbox {{\boldmath $\theta$}}}
\newcommand{\zz}{\vect{z}}

\renewcommand{\TH}{\vect{\Theta}}

%\newcommand{\at}{{\alpha_t}}
\newcommand{\At}{\vect{\alpha}_t}
\newcommand{\aq}{\alpha_q}
\newcommand{\atq}{\at^q}
\newcommand{\atmq}{\a_{t-1}^q}
\newcommand{\btq}{\beta_t^q}

\newcommand{\e}{\eta}
%\newcommand{\eb}{\eta_B}
\newcommand{\ebi}{\e_B^{-1}}
\newcommand{\et}{\e_t}
\newcommand{\eT}{\e_T}
\newcommand{\eo}{\e_1}
\newcommand{\eoo}{\e_2}
\newcommand{\etp}{\e_{t+1}}
\newcommand{\eTp}{\e_{T+1}}
\newcommand{\etpp}{\e_{t+2}}
\newcommand{\eTpp}{\e_{T+2}}
\newcommand{\etm}{\e_{t-1}}
\newcommand{\eti}{\et^{-1}}
\newcommand{\eoi}{\eo^{-1}}
\newcommand{\eooi}{\eoo^{-1}}
\newcommand{\etpi}{\etp^{-1}}
\newcommand{\eTpi}{\eTp^{-1}}
\newcommand{\etppi}{\etpp^{-1}}
\newcommand{\eTppi}{\eTpp^{-1}}
\newcommand{\etmi}{\etm^{-1}}
\newcommand{\es}{\squiggle{\e}}

\renewcommand{\I}{\vect{I}}

\newcommand{\E}{\vect{\e}}
\newcommand{\Ei}{\E^{-1}}
%\newcommand{\Eb}{\E_B}
\newcommand{\Et}{\E_t}
\newcommand{\ET}{\E_T}
\newcommand{\Eo}{\E_1}
\newcommand{\Etp}{\E_{t+1}}
\newcommand{\Eti}{\Et^{-1}}
\newcommand{\Eoi}{\Eo^{-1}}
\newcommand{\Etpi}{\Etp^{-1}}
\newcommand{\Ebi}{\E_B^{-1}}
\newcommand{\Es}{\squiggle{\E}}

\renewcommand{\at}{\a_t}
\newcommand{\atp}{\a_{t+1}}

\newcommand{\pred}{{\hat{a}}}
\newcommand{\predt}{{\pred_t}}

\newcommand{\Q}{\Phi}
%\newcommand{\q}{\phi}

\renewcommand{\z}{\vect{z}}
\newcommand{\zs}{\tilde{\z}}
\renewcommand{\r}{\vect{r}}

\newcommand{\lt}{{L_t}}
\newcommand{\lot}{{L_{1..t}}}
\newcommand{\loT}{{L_{1..T}}}
\newcommand{\lotm}{{L_{1..t-1}}}
\renewcommand{\lq}{{L_q}}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}


==> tex/relatedwork.tex <==

\section{Related Work}

%The development of SG-MCMC algorithms has popularized large-scale Bayesian learning in modern
%machine learning such as deep learning \cite{ChenDC:NIPS15}. pSGD-AM extends an arguably most 
%expressive SG-MCMC algorithm, the multivariate stochastic gradient Nos\'{e}-Hoover 
%thermostat \cite{GanCHCC:icml15}, for stochastic optimization. Related MCMC algorithms for global 
%optimization has been studied in the framework of {\em simulated 
%annealing} \cite{Kirkpatrick:science83,Cerny:JOTA85}. However, little work has been done in the context of 
%SG-MCMC algorithms.

The idea of annealing system temperature is from the {\em simulated annealing} \cite{Kirkpatrick:science83,Cerny:JOTA85},
which was later extended, for example, in the framework of reversible jump MCMC \cite{AndrieuFD:UAI00},
annealing important sampling \cite{Neal:SC01} and parallel tempering \cite{LiPAZG:AMC09}. These works are based on
the Metropolis--Hastings algorithm, which is computationally infeasible in large-scale learning but not required in Santa. 
By considering minibatches of data in each iteration, {\em subsample annealing} algorithms has been 
proposed \cite{VandeMeentPW:arx14,ObermeyerGJ:AISTATS14}. The proposed Santa differs from all the 
above algorithms in that it serves as the first work built upon the recently developed SG-MCMC framework
for stochastic optimization.

Santa, in the temperature limit, closely relates to the SGD with momentum algorithm \cite{RumelhartHW:nature86},
except that both gradient and momentum are updated adaptively.
Other related stochastic optimization algorithms include the stochastic gradient descend (SGD) \cite{Bottou:book98}, 
RMSprop \cite{tieleman2012lecture}, Adagrad \cite{duchi2011adaptive},
Adadelta \cite{zeiler2012adadelta} and the recently proposed Adam algorithm \cite{kingma2014adam}. 
Adaptive momentum is a new feature in Santa that is lack of in existing stochastic optimization algorithms.
More importantly, different from the above mentioned algorithms, convergence analysis suggests that Santa is able
to find a solution close to the global optima for an (non-convex) optimization problem, which is
infeasible for existing stochastic optimization algorithms.



==> tex/theory.tex <==
\vspace{-0.1cm}\section{Theoretical Foundation}\label{sec:theory}
In this section we present the stochastic differential equations (SDEs) that correspond to the SANTA algorithm.
The SDEs are presented with re-parameterized with $\pb = \ub / \eta^{1/2}$, $\Xib = \alphab / \eta^{1/2}$, as in \cite{DingFBCSN:NIPS14}.
The SDEs describes a particle in a physical system with $\thetab$ being the location and $\pb$ 
the momentum of a particle.
%In the SDEs, following \cite{DingFBCSN:NIPS14}, reparameterized momentum and thermostat variables
%for those in Algorithm~\ref{alg:sahmc} are used, {\it e.g.},
%$\pb = \ub / \eta^{1/2}$, $\Xib = \alphab / \eta^{1/2}$.
We develop theory on convergence properties using tools from the SDE literature, extending mSGNHT theory \cite{DingFBCSN:NIPS14,GanCHCC:icml15}.
%which describes the motion of particles in a physical system with $\thetab$ being to the location and $\pb$ 
%the momentum of the particle.

The particle is driven by a random force $\tilde{\fb}_t \triangleq -\nabla_{\thetab}\tilde{U}_t(\thetab)$ at time $t$.
The stationary distribution of $\thetab$ corresponds to the model posterior of interest \cite{GanCHCC:icml15}.
Our critical extension is the use of Riemannian information geometry, critical for fast convergence \cite{PattersonT:NIPS13}.
The system is described by the following SDEs\footnote{With a little bit abuse of notation but for conciseness, 
in this paper $\nabla_{\thetab}\Gb(\thetab)$ denotes a vector with the $i$-th element being 
$\sum_j \nabla_{\thetab_i}\Gb_{ij}(\thetab)$.}:


%In this section, we develop theory using tools from stochastic different equations to support the pSGD-AM algorithm, 
%as well as its convergence properties, using tools from stochastic different equations.
%Different from conventional stochastic optimzation algorithms, pSGD-AM is built upon a recently
%proposed SG-MCMC algorithm call the multivariate stochastic gradient 
%thermostat (mSGNHT) \cite{DingFBCSN:NIPS14,GanCHCC:icml15}.
%mSGNHT describes motion of particles in a physical system where the model parameter $\thetab$ corresponds 
%to the location variable. Particles in the system are driven by a random force
%$\tilde{f}_t(\thetab) \triangleq -\nabla_{\thetab}\tilde{U}_t(\thetab)$ at time $t$. The stationary distribution of the 
%location variable $\thetab$ can be shown to coincide with the model posterior of interest \cite{GanCHCC:icml15}. 
%In pSGD-AM, we extend mSGNHT by incorporating Riemannian information geometry (characterized by some 
%Riemannian metrics) into the system, which has proven critical for fast convergence \cite{PattersonT:NIPS13}.
%The system is described by the following SDEs:
%\begin{align}\label{eq:srhmc1}
%	&\left\{\begin{array}{ll}
%	\mathrm{d}\theta &= G(\theta)^{-1}p \mathrm{d}t \\
%	\mathrm{d}p &= \left(-G(\theta)^{-1}\nabla_\theta U(\theta) - \Xi p + \nabla_\theta G(\theta)^{-1}\right) \mathrm{d}t + \sqrt{2C}\mathrm{d}W \\
%	\mathrm{d}\Xi &= \left(q - I\right)\mathrm{d}t
%	\end{array}\right.
%\end{align}
%where $q = \mbox{diag}(p^2)$, $U(\theta)$ is the negative log-posterior, $C > 0$ is a constant, $W$ is standard Brownian motion.
%Or a more general version:
\vspace{-0.4cm}
\begin{align}\label{eq:srhmc2}
	&\left\{\begin{array}{ll}
	\mathrm{d}\thetab &= \Gb_1(\thetab)\pb \mathrm{d}t \\
	\mathrm{d}\pb &= \left(-\Gb_1(\thetab)\nabla_\thetab U(\thetab) - \Xib \pb + \nabla_\thetab \Gb_1(\thetab)\right. \\
	 & \hspace{-0.7cm}\left.- \Gb_1(\thetab)(\Xib - \Gb_2(\thetab))\nabla_{\thetab}\Gb_2(\thetab)\right) \mathrm{d}t + \sqrt{2\Gb_2(\thetab)}\mathrm{d}W \\
	\mathrm{d}\Xib &= \left(\mbox{diag}(\pb\odot \pb) - I\right)\mathrm{d}t
%	\mathrm{d}\Xib &= \left(\Qb - I\right)\mathrm{d}t
	\end{array}\right.
\end{align}
%where $\Qb = \mbox{diag}(\pb\odot \pb)$ with $\pb \in \RR^p$ being momentum variables, 
$W$ is standard Brownian motion. 
$\Gb_1(\thetab)$ encodes geometric information of the potential energy $U(\thetab)$, 
and $\Gb_2(\thetab)$ characterizes the manifold geometry of the Brownian motion. 
Note $\Gb_2(\thetab)$ may be the same as $\Gb_1(\thetab)$ for the same Riemannian manifold. 
We call $\Gb_1(\thetab)$ and $\Gb_2(\thetab)$ Riemannian metrics, 
which are commonly defined by the Fisher information matrix \cite{GirolamiC:JRSSB11}. 
We use the RMSprop preconditioner approximation (with updates from Algorithm~\ref{alg:sahmc}) for computational feasibility.
%However we use preconditioners constructed from the RMSprop algorithm in Algorithm~\ref{alg:sahmc} for computational feasibility. 
Using the Fokker-Plank equation \cite{Risken:FPE89}, we show that the marginal stationary distribution of \eqref{eq:srhmc2} corresponds to the posterior distribution.

\begin{lemma}\label{lem:FP}
	Denote $\Ab:\Bb \triangleq \mbox{tr}\left\{\Ab^T\Bb\right\}$.The stationary distribution of \eqref{eq:srhmc2} is:
	$p(\thetab, \pb, \Xib) \propto$
	\begin{align*}
		\exp\left\{-U(\thetab) + \frac{1}{2}\pb^T\pb
		+ \frac{1}{2}\left(\Xib - G_2(\thetab)\right):\left(\Xib - G_2(\thetab)\right)\right\}~.
	\end{align*}
\end{lemma}
{\color{red} Is there a proof somewhere?}

We note that $\pb$ in \eqref{eq:srhmc2} has additionally dependencies on $\Gb_1$ and $\Gb_2$ compared to \cite{GanCHCC:icml15}. 
$\Xib \pb$ introduces friction into the system so that the particle would not move too far away by the random force;
the other two terms with $\nabla_{\thetab}G_1(\thetab)$ and $\nabla_{\thetab}G_2(\thetab)$ penalize the influences of the Riemannian metrics so that the stationary distribution remains invariant.

%By looking at the SDE for $\pb$ in \eqref{eq:srhmc2}, it is interesting to see that in addition to the terms containing 
%gradient and Brownian motion, extra terms with $\Gb_1$ and $\Gb_2$ are also presented. These terms 
%essentially penalize the influences of the Riemannian metrics, so that the stationary distribution of the system remains invariant. 
%Specifically, $\Xib \pb$ is called the friction term, 
%which introduces friction into the system so that the particle would not move too far away by the random force; the other two 
%terms with $\nabla_{\thetab}G_1(\thetab)$ and $\nabla_{\thetab}G_2(\thetab)$ essentially prevent the 
%stationary distribution distorted by applying the geometric information to the gradient and Brownian motion terms
%in \eqref{eq:srhmc2}, respectively.

\subsection{Exploration}
The first stage of SANTA, {\em exploration} explores the parameter space to obtain parameters near the global mode objective function\footnote{This requires an ergodic algorithm. 
While ergodicity is not straightforward to check on objective functions of interest, we follow most MCMC literatures and assumes it holds in our algorithm.}.
This approach applies ideas from simulated annealing \cite{Kirkpatrick:science83}. 
Specifically, an inverse temperature $\beta$ is introduced into the SDE \eqref{eq:srhmc2}. 
It is slowly annealed to temperature zero to freeze the particles at the global mode. 
To this end, we propose the following SDE system with temperatures based on \eqref{eq:srhmc2}:

\begin{align}\label{eq:srhmc3}
%	&H = \beta \left(U(\theta) + \frac{1}{2}p^Tp + \frac{1}{2}(\Xi - G_2(\theta)):(\Xi - G_2(\theta))^T\right) \nonumber\\
	&\left\{\begin{array}{ll}
	\mathrm{d}\thetab &= G_1(\thetab)\pb \mathrm{d}t \\
	\mathrm{d}\pb &= \left(-G_1(\thetab)\nabla_\thetab U(\thetab) - \Xib \pb + \frac{1}{\beta}\nabla_\thetab G_1(\thetab)\right. \\
	 &\hspace{-0.6cm}\left.+ G_1(\thetab)(\Xib - G_2(\thetab))\nabla_{\thetab}G_2(\thetab)\right) \mathrm{d}t + \sqrt{\frac{2}{\beta}G_2(\thetab)}\mathrm{d}W \\
	\mathrm{d}\Xib &= \left(\qb - \frac{1}{\beta}I\right)\mathrm{d}t~.
	\end{array}\right.
\end{align}
As in Lemma~\ref{lem:FP}, the stationary distribution of \eqref{eq:srhmc3} can be proved to be:
\begin{align}\label{eq:staitonary_beta}
	p(\thetab, \pb, \Xib) \propto e^{-\beta U(\thetab) + \frac{\beta}{2}\pb^T\pb
	+ \frac{\beta}{2}\left(\Xib - G_2(\thetab)\right):\left(\Xib - G_2(\thetab)\right)}~.
\end{align}\vspace{-0.5cm}

Notice that minimizing $U(\thetab)$ is equivalent to sampling from 
$p(\thetab) \triangleq \frac{1}{Z}e^{-\beta U(\thetab)}$ (proportional to \eqref{eq:staitonary_beta})
in the zero-temperature limit $\beta \rightarrow \infty$, {\it i.e.},
$\{\thetab^* = \arg\!\min U(\thetab)\} \equiv \{\thetab^* \sim \lim_{\beta \rightarrow \infty}\frac{1}{Z}e^{-\beta U(\thetab)}\}$.
Here $Z$ is the normalization constant such that $p(\thetab)$ is a valid distribution.
Based on this, it is ready to construct a Markov chain
that sequentially transits from high temperatures to low temperatures. At the state equilibrium, the chain 
would reach the temperature limit with marginal stationary distribution
$\rho_0(\thetab) \triangleq \lim_{\beta \rightarrow \infty}\frac{1}{Z}e^{-\beta U(\thetab)}$, a point mass locating
at the global mode of $U(\thetab)$. Specifically, we first define a sequence of 
inverse temperatures, $(\beta_1, \beta_2, \cdots, \beta_L)$, such that $\beta_L$ is large enough\footnote{Due to numerical 
issues, it is impossible to set $\beta_L$ to be infinite, we thus assign a large enough value for it and handle the infinity case in the {\em refinement step} in the second stage of the algorithm.}.
For each time $t$, we generate a sample according to the SDE system \eqref{eq:srhmc3} with temperature $\frac{1}{\beta_t}$, 
conditioned on the sample from the previous temperature, $\frac{1}{\beta_{t-1}}$. 
Analogy to the simulated annealing, we call this procedure annealing thermostats. The problem now translates to
generating highly accurate samples from \eqref{eq:srhmc3}, which is addressed in the next section.

%\begin{align}\label{eq:srhmc4}
%	&H = \beta U(\theta) + \frac{1}{2}p^Tp + \frac{1}{2}(\Xi - \frac{1}{\beta}G_2(\theta)):(\Xi - \frac{1}{\beta}G_2(\theta))^T \nonumber\\
%	&\left\{\begin{array}{ll}
%	\mathrm{d}\theta &= G_1(\theta)p \mathrm{d}t \\
%	\mathrm{d}p &= \left(-\beta G_1(\theta)\nabla_\theta U(\theta) - \Xi p + \nabla_\theta G_1(\theta) + \frac{1}{\beta}G_1(\theta)(\Xi - \frac{1}{\beta}G_2(\theta))\nabla_{\theta}G_2(\theta)\right) \mathrm{d}t + \sqrt{\frac{2}{\beta}G_2(\theta)}\mathrm{d}W \\
%	\mathrm{d}\Xi &= \left(q - I\right)\mathrm{d}t
%	\end{array}\right.
%\end{align}

\paragraph{Generating approximate samples}\label{para:SSI}

Generating exact samples from the SDE \eqref{eq:srhmc3} is infeasible for general models. 
As a result, we resort to numerical methods for generating approximate samples. 
The most popular numerical integrator is the Euler scheme, which results in Algorithm~\ref{alg:sahmc}. 
However, Euler scheme is a 1st-order method thus approximation
errors are relatively high \cite{ChenDC:NIPS15}. To generate more accurate samples, we resort to an
easily implemented 2nd-order symmetric splitting scheme (SSS) \cite{ChenDC:NIPS15}.
The idea of SSS is to split an infeasible SDE into several sub-SDEs, with each part analytically solvable;
approximate samples are then generated by sequentially evolving parameters via these sub-SDEs. 
Specifically, in SANTA, we split \eqref{eq:srhmc3} into the following three sub-SDEs:
\begin{align*}%\label{eq:split_sghmc}
	&A: \left\{\begin{array}{ll}
	\mathrm{d}\thetab &= \Gb_1(\thetab)\pb \mathrm{d}t \\
	\mathrm{d}\pb &= 0 \\
	\mathrm{d}\Xi &= \left(\qb - \frac{1}{\beta}I\right)\mathrm{d}t
	\end{array}\right.,
	B: \left\{\begin{array}{ll}
	\mathrm{d}\thetab &= 0 \\
	\mathrm{d}\pb &= - \Xib \pb \mathrm{d}t \\
	\mathrm{d}\Xib &= 0
	\end{array}\right., \\
	&O: \left\{\begin{array}{ll}
	\mathrm{d}\thetab &= 0 \\
	\mathrm{d}\pb &= \left(-G_1(\thetab)\nabla_\thetab U(\thetab) + \frac{1}{\beta}\nabla_\thetab G_1(\thetab)\right. \\ 
	 &\hspace{-1cm}\left.+ G_1(\thetab)(\Xib - G_2(\thetab))\nabla_{\thetab}G_2(\thetab)\right) \mathrm{d}t + \sqrt{\frac{2}{\beta}G_2(\thetab)}\mathrm{d}W \\
	\mathrm{d}\Xib &= 0
	\end{array}\right. \nonumber
\end{align*}

We then use the order ABOBA to show the above sub-SDEs to generate approximate
samples \cite{ChenDC:NIPS15}, with update equations given in
the appendix. Specifically, based on the splitting, parameters first evolve
following $A$ for time $h/2$, then $B$ for time $h/2$, $C$ for time $h$, 
$B$ again for time $h/2$, and finally $A$ again for time $h/2$, resulting in 
the update equations in Algorithm~\ref{alg:sahmc_ssi}. Here $h$ represents the 
stepsize\footnote{Using the reparameterization in \cite{DingFBCSN:NIPS14}, we have $h = \sqrt{\eta}$ for $\eta$ defined 
in Algorithm~\ref{alg:sahmc}.}. The resulting parameters then serve as an approximate sample from
the SSS. When replacing $\Gb_1$ and $\Gb_2$ with preconditioners constructed from the RMSprop,
we arrive at Algorithm~\ref{alg:sahmc_ssi}. Note the terms $\nabla_{\thetab}G_1(\thetab)$ and $\nabla_{\thetab}G_2(\thetab)$
in the above split SDEs are not straightforward to calculate, we propose an approximation for it in the next section.

\paragraph{Approximate calculation for $\nabla_{\thetab}\Gb_1(\thetab)$}\label{sec:gradient_app}

We proposes a computationally efficient approximation for calculating $\nabla_{\thetab}\Gb_1(\thetab)$ 
based on the definition of derivatives. Specifically, for $\nabla_{\thetab}\Gb_1(\thetab)$ at the $t$-th iteration, 
denoted as $\nabla_{\thetab}\Gb_1^t(\thetab)$, it is approximated as:
\begin{align*}
	\nabla_{\thetab}\Gb_1^t(\thetab) &\stackrel{A_1}{\approx} \frac{\Gb_1^t(\thetab) - \Gb_1^{t-1}(\thetab)}{\thetab_t - \thetab_{t-1}} \\
	&\stackrel{A_2}{=} \frac{\Gb_1^t(\thetab) - \Gb_1^{t-1}(\thetab)}{\Gb_1^t(\thetab)\pb_{t-1} h} = \frac{1}{\ub_{t-1}}\left(1 - \frac{\Gb_1^{t-1}(\thetab)}{\Gb_1^t(\thetab)}\right)
\end{align*} 
where $A_1$ follows by the definition of derivatives, $A_2$ by using the update equation for
$\thetab_t$, {\it i.e.}, $\thetab_t = \thetab_{t-1} + \Gb_1^t(\thetab)\pb_{t-1} h$.
According to the Taylor theory, the approximation error above is in the order of $O(h)$, {\it e.g.},
\begin{align}\label{eq:approx_grad}
	\left\|\frac{\Gb_1^t(\thetab) - \Gb_1^{t-1}(\thetab)}{\Gb_1^t(\thetab)\pb_t h} - \nabla_{\thetab}\Gb_1^t(\thetab)\right\| \leq \mathcal{B}_t h~,
\end{align}
for some positive constant $\mathcal{B}_t$. It is interesting to see that the approximation error is negligible in term of 
convergence behaviors because the error can be absorbed into the errors from stochastic gradients. 
Formal theoretical analysis on convergence behaviors with this approximation will be given in later sections. 
Using similar tricks, $\nabla_{\thetab}G_2^t(\thetab)$ can also be approximatly calculated.
This completes computation for the {\em exploration} stage in Algorithm~\ref{alg:sahmc}.

\subsection{Refinement}

The {\em refinement} stage corresponds to the zero-temperature limit for the {\em exploration} stage.
In this section we show that in the zero-temperature limit, the updates in the
{\em exploration} stage can be significantly simplified, leading to an SGD with momentum like 
stochastic optimization algorithm.

Specifically, it is reasonable to assume that the Markov chain has reached its equilibrium after the {\em exploration} stage.
Now we show that in the zero-temperature limit, some terms in the 
SDE \eqref{eq:srhmc3} vanish. First, as $\beta \rightarrow \infty$, the term 
$\frac{1}{\beta}\nabla_{\thetab}\Gb_1(\thetab)$ and the variance term for the Brownian motion are easily seen approaching 0; 
second, in the equilibrium state, from the stationary
distribution \eqref{eq:staitonary_beta}, the thermostat variable $\Xib$ approaches $\Gb_2(\thetab)$, thus the term
$\Gb_1(\thetab)(\Xib - \Gb_2(\thetab))\nabla_{\thetab}\Gb_2(\thetab)$ vanishes; similarly, from \eqref{eq:staitonary_beta},
we have $\mathbb{E}\qb_i \triangleq \mathbb{E}\pb_i^2 \rightarrow 0$, this makes the
SDE for $\Xib$ in \eqref{eq:srhmc3} vanish as well. As a result, in the {\em refinement} stage, only $\thetab$ and
$\pb$ are updated. When using the symmetric splitting scheme to solve the corresponding SDEs, it results
in the update equations in Algorithm~\ref{alg:sahmc_ssi}.

\paragraph{Relation with other stochastic optimization algorithms}
The relation between SANTA in the {\em refinement} stage and other representative stochastic optimization
algorithms can be seen more clearly from Algorithm~\ref{alg:sahmc} using the Euler scheme. 
Compared with SGD-Moment \cite{RumelhartHW:nature86}, SANTA provides mechanisms for both adaptive gradient and adaptive 
momentum updates. Furthermore, different from adaptive gradient algorithms such as Adagrad \cite{duchi2011adaptive} 
and RMSprop \cite{tieleman2012lecture}, SANTA is a momentum based algorithm. Finally, when compared with 
a recently proposed ADAM algorithm \cite{kingma2014adam}, SANTA provides a principle way to update
momentum variables element-wise. For the reasons, SANTA serves as a more general stochastic optimization 
algorithm than existing ones.

\subsection{Convergence properties}
We study the convergence properties of SANTA in this section, based on the framework developed
in \cite{ChenDC:NIPS15}. We will first focus on the {\em exploration} stage of the algorithm. By using the
Monotone Convergence argument, convergence for the {\em refinement} stage can be obtained by taking 
the temperature limit from the results of the {\em exploration} stage. Distinct from conventional stochastic
optimization algorithms, we prove that 
SANTA finds a solution to an (non-convex) optimization problem that is close to its global optima.

Formally, the goal of SANTA is to find $\thetab^*$ such that $\thetab^* = \arg\!\min_{\thetab} U(\thetab)$.
Let $\{\thetab_1, \cdots, \thetab_L\}$
be a sequence of parameters collected from the algorithm. 
Define $\hat{U} \triangleq \frac{1}{L}\sum_{t=1}^L U(\thetab_t)$ as the
sample average, $\bar{U} \triangleq U(\thetab^*)$ the global optima of $U(\thetab)$.
In the following we develop theory to measure the closeness of $\hat{U}$ and the global optima $\bar{U}$.

Before presenting the theory, we follow the framework for general SG-MCMC \cite{ChenDC:NIPS15}, to make certain 
assumptions on the potential energy $U$. First, we defined a functional $\psi_t$ for each $t$ that solves the following 
Poisson equation:
\begin{align}\label{eq:PoissonEq1}
	\mathcal{L}_t \psi_t(\thetab_{t}) =  U(\thetab_{t}) - \bar{U}~,
\end{align}
where $\mathcal{L}_t$ is the generator of the SDE system \eqref{eq:srhmc3} for the $t$-th iteration, defined as
$\mathcal{L}_tf(\Xb_t) \triangleq \lim_{h \rightarrow 0^{+}} \frac{\mathbb{E}\left[f(\Xb_{t+h})\right] - f(\Xb_t)}{h}$
with $\Xb_t \triangleq (\thetab_t, \pb_t, \Xib_t)$, $f: \RR^{3p} \rightarrow \RR$ a compactly supported twice differentiable function.
The solution functional $\psi_t(\thetab_{t})$ characterizes the difference between $U(\thetab_{t})$ 
and the global optima $\bar{U}$ for every $\thetab_{t}$. As shown in \cite{MattinglyST:JNA10}, \eqref{eq:PoissonEq1} 
typically possesses a unique solution, which is at least as smooth as $U$ under the elliptic or hypoelliptic settings.
Our assumption is on the boundedness and smoothness of $\psi_t$, described in 
Assumption~\ref{ass:assumption1}.

\begin{assumption}\label{ass:assumption1}
$\psi_t$ and its up to 3rd-order derivatives, $\mathcal{D}^k \psi_t$, are bounded by a
function $\mathcal{V}(\thetab, \pb, \Xib)$, {\it i.e.}, 
$\|\mathcal{D}^k \psi\| \leq C_k\mathcal{V}^{r_k}$ for $k=(0, 1, 2, 3)$, $C_k, r_k > 0$. Furthermore, 
the expectation of $\mathcal{V}$ is bounded: $\sup_t \mathbb{E}\mathcal{V}^r(\thetab, \pb, \Xib) < \infty$, 
and $\mathcal{V}$ is smooth such that 
$\sup_{s \in (0, 1)} \mathcal{V}^r\left(s\Xb + \left(1-s\right)Y\right) \leq C\left(\mathcal{V}^r\left(\Xb\right) + \mathcal{V}^r\left(Y\right)\right)$, $\forall \Xb \in \RR^{3p}, Y \in \RR^{3p}, r \leq \max\{2r_k\}$ for some $C > 0$.
\end{assumption}

Let $\Delta U(\thetab) \triangleq U(\thetab) - U(\thetab^*)$. Further define an operator 
$\Delta V_t = \left(G_1(\thetab)(\nabla_{\thetab}\tilde{U}_t - \nabla_{\thetab} U) + \frac{\mathcal{B}_t}{\beta_t}\right) \cdot \nabla_{\pb}$
for each $t$, where $\mathcal{B}_t$ is from \eqref{eq:approx_grad}. Theorem~\ref{theo:bias1} depicts the closeness of $\hat{U}$ to
the global optima $\bar{U}$ in term of {\em bias} and {\em mean square error} (MSE) defined below.

\begin{theorem}\label{theo:bias1}
	Under Assumption~\ref{ass:assumption1}, let $\left\|\cdot\right\|$ be the operator norm.
	The bias and MSE of the {\em exploration} stage in SANTA with respect to the global optima for $L$ steps
	with stepsize $h$ is bounded, for some constants $C > 0$ and $D > 0$, as:
	{\small\begin{align*}
		\mbox{Bias: }&\left|\mathbb{E}\hat{U} - \bar{U}\right| \leq C\left|U(\thetab^*)\right|\left(\frac{1}{L}\sum_{t=1}^L\int e^{-\beta_t\Delta U(\thetab)}\mathrm{d}\thetab\right) \\
		&~~~~~~~~~~~~~~~+ D\left(\frac{1}{Lh} + \frac{\sum_t \left\|\mathbb{E}\Delta V_t\right\|}{L} + h^2\right)~. \\
	\mbox{MSE: }&\mathbb{E}\left(\hat{U} - \bar{U}\right)^2 \leq C^2U(\thetab^*)^2\left(\frac{1}{L}\sum_{t=1}^L\int e^{-\beta_t\Delta U(\thetab)}\mathrm{d}\thetab\right)^2 \\
		&~~~~~~~~~~~~~~~+ D^2 \left(\frac{\frac{1}{L}\sum_t\mathbb{E}\left\|\Delta V_t\right\|^2}{L} + \frac{1}{Lh} + h^{4}\right)~.
	\end{align*}}
\end{theorem}

%\begin{theorem}\label{theo:MSE}
%	Under Assumptions~\ref{ass:assumption1}, the MSE of the {\em exploration} stage in pSGD-AM with 
%	respect to the global optima for $L$ steps with stepsize $h$ is bounded,
%	for some constants $C > 0$ and $D > 0$, as
%	\begin{align*}
%		\mathbb{E}\left(\hat{U} - \bar{U}\right)^2 &\leq CU(\thetab^*)^2\left(\frac{1}{L}\sum_{t=1}^L\int e^{-\beta_t\Delta U(\thetab)}\mathrm{d}\thetab\right)^2 \\
%		&+ D \left(\frac{\frac{1}{L}\sum_t\mathbb{E}\left\|\Delta V_t\right\|^2}{L} + \frac{1}{Lh} + h^{4}\right)~.
%	\end{align*}
%\end{theorem}
From Theorem~\ref{theo:bias1}, it can be seen that the bias and MSE bounds share similar forms as convergence results
for general SG-MCMC algorithms \cite{ChenDC:NIPS15}, except the additional integration terms,
which decrease to zero exponentially fast. Furthermore, the term $\frac{\sum_t \left\|\mathbb{E}\Delta V_t\right\|}{L}$
in the bias would vanish as long as the sum of the annealing sequence $\{\beta_t\}$ is finite\footnote{In practice we might
not need to care about this constraint because a little bit bias in the {\em exploration} stage does not affect convergence of
the {\em refinement} stage.}, indicating that the gradient
approximation for $\nabla_{\thetab}G_1(\thetab)$ in Section~\ref{sec:gradient_app} does not affect the bias of the algorithm. 
Similar arguments apply for the MSE bound. 

To get convergence results for the {\em refinement} stage, let a sequence
of functions $\{g_m\}$ be defined as $g_m \triangleq -\frac{1}{L}\sum_{l=m}^{L+m-1} e^{-\beta_l\hat{U}(\thetab)}$,
it is easy to see the sequence $\{g_m\}$ satisfies $g_{m_1} < g_{m_2}$ for $m_1 < m_2$, and $\lim_{m \rightarrow \infty} g_m = 0$. 
According to the Monotone Convergence Theorem, the bias and MSE in
the zero-temperature limit exists. This leads to
the following convergence results for the {\em refinement} stage.

\begin{corollary}\label{coro:refine_con}
	Under Assumptions~\ref{ass:assumption1}, the bias and MSE of the {\em refinement} stage in SANTA with 
	respect to the global optima for $L$ steps with stepsize $h$ are bounded, for some constants 
	$D_1 > 0$, $D_2 > 0$, as
	\begin{align*}
		\mbox{Bias: }&\left|\mathbb{E}\hat{U} - \bar{U}\right| \leq D_1\left(\frac{1}{Lh} + \frac{\sum_t \left\|\mathbb{E}\Delta V_t\right\|}{L} + h^2\right) \\
		\mbox{MSE: }&\mathbb{E}\left(\hat{U} - \bar{U}\right)^2 \leq D_2 \left(\frac{\frac{1}{L}\sum_t\mathbb{E}\left\|\Delta V_t\right\|^2}{L} + \frac{1}{Lh} + h^{4}\right)
	\end{align*}
\end{corollary}

Corollary~\ref{coro:refine_con} share similar  bounds as those for general
SG-MCMC \cite{ChenDC:NIPS15}, thus the convergence rates are the same as SG-MCMC, {\it e.g.} $L^{-4/5}$ in
term of the MSE, which is slower than standard SGD algorithm. However, these are convergence rates for the bounds. 
In practice, we still find as fast convergence of SANTA as other stochastic optimization algorithms.

